High Resolution Generation Expansion Planning Considering Flexibility Needs: The Case of Switzerland in 2030

This paper presents a static generation expansion planning formulation in which operational and investment decisions for a wide range of technologies are co-optimized from a centralized perspective. The location, type and quantity of new generation and storage capacities are provided such that system demand and flexibility requirements are satisfied. Depending on investments in new intermittent renewables (wind, PV), the flexibility requirements are adapted in order to fully capture RES integration costs and ensure normal system operating conditions. To position candidate units, we incorporate DC constraints, nodal demand and production of existing generators as well as imports and exports from other interconnected zones. To show the capabilities of the formulation, high-temporal resolution simulations are conducted on a 162-bus system consisting of the full Swiss transmission grid and aggregated neighboring countries.

==> exports_imports_2030.tex <==
\begin{table}[htb!]
	\centering
	\caption{Net CH cross-border exchange 2015 vs. 2030 (sim.)}
	\vspace{0.2cm}
	\label{exports imports2030}
	\renewcommand{\arraystretch}{1.1}
	\begin{tabular}{ccc}%|m{13mm}|}
		\hline
		\textbf{Net Export (From - To)} & \textbf{BaU [TWh]} & \textbf{RES [TWh]} %& \textbf{Constraints}%
		\\
		\hline
		AT - CH  & 5.3 & 5.1 %& \vspace{1mm} \eqref{eq:thermal reserves1} - \eqref{eq:thermal reserves4}%
		\\
		%\hline
		DE - CH & 5.6 & 3.4
		\\
		%\hline
		FR - CH & 20.7 & 20.3
		\\
		%\hline
		CH - IT & 22.0 & 22.9
		\\
		\hline
	\end{tabular}
\end{table}
